A Resource-Free Evaluation Metric for Cross-Lingual Word Embeddings Based on Graph Modularity

Cross-lingual word embeddings encode the meaning of words from different languages into a shared low-dimensional space. An important requirement for many downstream tasks is that word similarity should be independent of language - i.e., word vectors within one language should not be more similar to each other than to words in another language. We measure this characteristic using modularity, a network measurement that measures the strength of clusters in a graph. Modularity has a moderate to strong correlation with three downstream tasks, even though modularity is based only on the structure of embeddings and does not require any external resources. We show through experiments that modularity can serve as an intrinsic validation metric to improve unsupervised cross-lingual word embeddings, particularly on distant language pairs in low-resource settings.

==> 60-related_work.tex <==
\section{Related Work}

%One line of work on evaluating cross-lingual embeddings is
%comparing their similarity with a fixed set of cross-lingual word pairs rated by
%humans~\citep{camacho2017semeval}, 
%but less work has focused on intrinsic measures 
%that correlate with downstream tasks. 
%One widely used intrinsic measure used to evaluate the coherence of
%monolingual embeddings is \textsc{qvec}~\citep{qvec:enmlp:15}. 
%\textsc{qvec} has been extended to use \abr{cca} (\textsc{qvec-cca}) 
%to output a score in $[-1, 1]$ to make the scores comparable across
%embeddings with different dimensions \citep{ammar2016massively}.
%However, while both \textsc{qvec} and \textsc{qvec-cca} can be extended for cross-lingual embeddings, 
%they are limited: they
%require external annotated corpora.  This is problematic in
%cross-lingual settings since this requires annotation to be consistent
%across languages~\citep{ammar2016massively}.

Our work is closest to \citet{eigenval_sim}. %\footnote{Per the author guidelines, 
They compute eigenvalue similarity between two monolingual lexical subgraphs built by subsampled words from two separate {\it monolingual} embeddings. % with a bilingual lexicon to obtain translation pairs. 
The resulting eigenvalue similarity has a high correlation with BLI on unsupervised cross-lingual embeddings obtained using MUSE~\cite{lample2018word}. 
In contrast, our cross-lingual lexical graph is directly derived from {\it cross-lingual} embeddings. % and explores three different cross-lingual embedding methods. 
Furthermore, we do not build subgraphs for samples of words, but rather consider the {\it entire} lexical graph. 
Finally, we explore the correlation with a classification task, 
which requires assumptions about the consistency across languages.

The cross-lingual embedding training methods that we consider all learn a single linear mapping from one embedding space to another, with different vector preprocessing steps and constraints~\cite{artetxe2018aaai}. 
Using a single linear mapping to map an entire embedding space to another is reported to be insufficient for correctly mapping all words from one language to another~\cite{P18-2036}. 
The underlying linearity of mapping is a potential cause of clustering by language, 
and we leave understanding how this property relates to modularity for future work.

%MP: This paragraph could be commented out if we need the space (but I would like to include it in the final version if so)
%Lastly, a related line of work is the intrinsic evaluation of probabilistic
%topic models, which are another low-dimensional representation of
%words and documents.  Metrics based on word co-occurrences
%have been developed for measuring the monolingual coherence of topics
%\citep{NewmanLGB10,MimnoWTLM11,LauNB14}. Less work has studied
%evaluation of cross-lingual topics \citep{MimnoWNSM09}. Some
%researchers have measured the overlap of direct translations across
%topics~\citep{Boyd-Graber:Blei-2009}, while \citet{Hao18mltm} propose
%a metric based on co-occurrences across languages that is more general
%than direct translations.



